WIPI: A New Web Threat for LLM-Driven Web Agents

With the fast development of large language models (LLMs), LLM-driven Web Agents (Web Agents for short) have obtained tons of attention due to their superior capability where LLMs serve as the core part of making decisions like the human brain equipped with multiple web tools to actively interact with external deployed websites. As uncountable Web Agents have been released and such LLM systems are experiencing rapid development and drawing closer to widespread deployment in our daily lives, an essential and pressing question arises: "Are these Web Agents secure?". In this paper, we introduce a novel threat, WIPI, that indirectly controls Web Agent to execute malicious instructions embedded in publicly accessible webpages. To launch a successful WIPI works in a black-box environment. This methodology focuses on the form and content of indirect instructions within external webpages, enhancing the efficiency and stealthiness of the attack. To evaluate the effectiveness of the proposed methodology, we conducted extensive experiments using 7 plugin-based ChatGPT Web Agents, 8 Web GPTs, and 3 different open-source Web Agents. The results reveal that our methodology achieves an average attack success rate (ASR) exceeding 90% even in pure black-box scenarios. Moreover, through an ablation study examining various user prefix instructions, we demonstrated that the WIPI exhibits strong robustness, maintaining high performance across diverse prefix instructions.

==> introduction.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\textwidth]{figures/webpipeline.pdf}
    \caption{Overview of practical black-box \wipi attack methodology.}
    \label{fig:webpipeline}
\end{figure*}


\section{Introduction}
% \fangzhou{TBD}
In recent years, we have witnessed the rapid development of \textit{Large Language Models} (LLMs). 
% From GPT2~\cite{radford2019language} to GPT3~\cite{brown2020language} and then to ChatGPT~\cite{chatgpt},
LLMs have drawn significant attention due to their remarkable capabilities and adaptability across a wide range of tasks, as evident in recent studies~\cite{pearce2022asleep, copilot, pearce2022examining, frieder2023mathematical,  lehnert2023ai, kortemeyer2023could}.  Among those LLMs, ChatGPT~\cite{chatgpt}, developed by OpenAI~\cite{openai}, stands out as the most popular and powerful player.
One of the most notable strengths of LLMs lies in their extraordinary language understanding and reasoning ability on diverse forms of textual information~\cite{chatgpt, touvron2023llama}. 
Consequently, taking advantage of that, there has been a proliferation of works dedicated to building various \textbf{LLM-driven systems} to carry out multiple tasks~\cite{zhou2023agents, wang2023voyager, park2023generative, xie2023openagents, chen2023agentverse, gozalo2023chatgpt, panda2023revolutionizing}. 
Among different LLM systems, those equipped with web tools to access and analyze resources from the Internet are usually called \textbf{Web Agents}. 
\wb can access and retrieve information from external websites. This feature enables LLM to read and analyze external webpages, and integrate up-to-date information. 
This enhances the capability of the LLM to generate more diverse and accurate information based on the retrieved content. 
% With this advanced capability, tons of \wb have been rapidly deployed into our daily life.
According to one of the most recent statistics~\cite {gptstore} in GPTs store, WebPilot (one of the most popular GPTs based \wb) has received over 100,000 visits within only one month. 
All these facts underscore the increasing integration of Web Agents into daily lives. 
% 100k+ web pilot

% \chaowei{why we need to study web agents? We need to have an argument here. }
As a specific type of LLM system, a Web Agent generally consists of a core LLM for information processing and extensional web tools for web resource retrieval.
To be specific, with the automatic LLM-driven working pipeline of Web Agents, the only thing that users need to do is input their instructions and target external URLs.
After receiving the instructions with external URLs from the user, the LLM will analyze the instructions and generate actions to call corresponding web tools, and then these tools will return the retrieved contents of the target webpages, which will be further analyzed by the LLM to generate the final response.
For instance, ChatGPT~\cite{chatgpt} can serve as a Web Agent when leveraging diverse web tools. Users can install plugins such as Web Pilot and Web Reader~\cite{reader, pilot} to enable them to access and summarize the content from external websites automatically. 

% For instance, in ChatGPT, users can utilize Web plugins such as Web Pilot and Web Reader~\cite{reader, pilot} to access and summarize the content from external websites automatically. 


% \shutong{Concept: LLM, Agent, system; need clarification. Btw, are LLM system and LLM Agent referring to the same concept?}
% \fangzhou{they are the same concept}


% Marked by the prosperity of diverse LLM-based Web Agents, the past year can be called the ``meta year'' of Web Agents. 
However, with the fast deployment of Web Agents into our real world, one fundamental question arises: ``Are these Web Agents secure?''
As an important part of the Internet, Web Agents bring convenience but also security risks.
Imagine a user trying to utilize a Web Agent like ChatGPT to access external web resources from the Internet, while some webpages released by an attacker are injected with some explicitly crafted prompts. After those malicious prompts are retrieved, LLMs would follow the attacker's instructions, being remotely compromised by the attacker.
We call this kind of indirect prompt injection that lurks inside the externally deployed webpages and targets Web Agents as \texttt{\textbf{W}eb \textbf{I}ndirect \textbf{P}rompt \textbf{I}njection (\textbf{WIPI})}, which is a brand-new type of web threat, different from either traditional web threats or existing prompt injection attacks targeted at only individual LLMs. 

% \shutong{WIP}
% Compared to traditional web threats, which are mainly brought by some malicious executable code inserted into the webpage, \wipi obtains better stealthiness. For instance, web norms can spread and steal private information via a specific part of its code. However, the driver of \wipi is the embedded indirect prompt in the format of natural language instead of executable code. Due to the flexibility of natural language (\emph{e.g.} paraphrasable and multilingual interpretation), and the indistinguishability between the injected prompt and the normal textual content, it is much harder for traditional web safeguards (like VirusTotal) to detect the existence of \wipi. 
% Second, there is no fixed pattern for WIPI. 
% Due to it consisting of natural languages and mixed with normal content of the webpage, the pattern of WIPI is not fixed. For instance, the same meaning of one English sentence can be interpreted in diverse language forms, and this sentence can be written in diverse languages, e.g., Spanish or Chinese. 
% Third, WIPI is more stealthy and less distinguishable. Indirect prompts are mixed with normal webpage content, which makes it hard to identify which part is indirect prompt or webpage content. Sometimes, indirect prompts can be appropriate to the theme of the homepage content, and when the content of the webpage is long, the identification becomes more challenging.

Previous studies on direct prompt injections~\cite{perez_ignore_2022, toyer_tensor_2023, pedro_prompt_2023, piet_jatmo_2024, yip_novel_2024, liu_prompt_2023} and 
Jailbreaks~\cite{jain2023baseline, deng2023jailbreaker, wei2023jailbroken, huang2023catastrophic, chao2023jailbreaking, yao2023fuzzllm} have revealed some vulnerabilities of LLMs. However, they do not pay much attention to the integrated LLM systems. Besides, the attacker has to the current user and is thus unable to bring any threats to others.
Yet, indirect prompt injections~\cite{greshake2023more, liu_prompt_2023-1, yi2023benchmarking} take a step forward and emerge as a significant system-level threat, and especially, Greshake et al. \cite{greshake2023more} point out that there could be threats of Indirect Prompt Injection when \wb accesses external sources. 
Nevertheless, all of those existing studies only stop at simple proof-of-concept experiments under offline datasets, lacking a thorough analysis and experiments of attacks in a real-world online setting. 
% aims to bypass the predefined rules and elect unexpected replies via directly injecting explicitly crafted prompts can be as one specific type of direct prompt injection.
% on LLM safety, involving the term ``Jailbreak'' that aims to bypass the predefined rules and elect unexpected replies via directly injecting explicitly crafted prompts, mainly focus on the core LLM. 
%% direct propmt injection
%%
% Although insightful, their limitations are also apparent, as the attacker is just the current user and cannot bring any threat to other users. 
% In addition, the integrated system is paid less attention and only some unexpected replies are far from bringing realistic security threats. 
% Indirect prompt injection, however, is a much more sophisticated and risky threat, as an attacker doesn't have to get involved in the conversation while being able to remotely control the LLM system in another user's session.
% and \textbf{they only care about ``Jailbreak'' in LLMs~\cite{wei2023jailbroken,deng2023jailbreaker} which cannot even be called as a security problem.} 
% Indirect prompt injection~\cite{greshake2023more, liu_prompt_2023-1, yi2023benchmarking} emerges as a significant threat to the LLM-driven systems.
% Greshake et al. \cite{greshake2023more} point out that there could be threats of Indirect Prompt Injection when \wb accesses the external sources. 
% Following this work, Yi et al. \cite{yi2023benchmarking} release a benchmark to evaluate the ability of current LLMs to defend against indirect prompt injections. 
% However, the vision of these works is also limited at the model level. The evaluation only leverages the local webpage dataset but fails to consider a more complicated and practical attack environment that includes real-world web tools.
% Greshake et al. \cite{greshake2023more} point out that there could be threats of indirect prompt injection in LLM-driven Web Agents. 
% Iqbal et al.~\cite{iqbal2023llm} take notable steps towards displaying the potential scenarios where attackers leverage compromised web tools to execute malicious operations. 
% However, they only stopped at simple proofs-of-concept, lacking a deep and practical analysis of the fundamental flaws in the real-world system.
% Yi et al. \cite{yi2023benchmarking} release a benchmark to evaluate the ability of current LLMs to defend against indirect prompt injections. 
% % However, its vision is also limited at the model level. The evaluation only leverages the local WebQA dataset but fails to conduct a more complicated and practical one that includes real-world web tools.
% Greshake et al. \cite{greshake2023more} point out that there could be threats of indirect prompt injection in LLM-driven Web Agents. 
% All of those existing studies only stop at simple proof-of-concept experiments under offline datasets, lacking a thorough analysis and experiments of real-world \wipi in a practical online setting. 
% complete pipeline of indirect prompt injection in an online setting and a deep and practical experiments in real-world \wb. 
% they don't provide , Besides, the experiments are conducted in an offline setting without any online web tools. 
% Hence it does not provide a deeper analysis combined with a practical Internet environment.
% The most recent work~\cite{} reveals three fundamental flaws in LLM systems and conducted real-world \wipi experiments via the web app version of ChatGPT. Additionally, it showcases several basic vulnerabilities in ChatGPT and a real-world attack scenario that can be directly deployed. However, the experimental setting is not practical and comprehensive enough, as the malicious webpage used in~\cite{} merely consists of indirect prompts without any normal content. 

% None of the existing works have ever tried to propose a practical and effective attack toward current real-world Web Agents, 
The limitations of existing works motivate us to propose a more comprehensive study of the attack on the practical threats of indirect prompt injections to LLM-driven Web Agents. 
Differently, starting from practicality, our proposed \wipi pipeline is targeted at the real-world deployed Web Agents. Specifically, our study considers the integrated system instead of individual modules, and an entirely online setting where accessible real-world webpages are off-site deployed. 
This requires us to consider the interactions between the core LLM and other different modules and the retrieving and processing of web resources via extensional tools.
Furthermore, we see the whole attacking pipeline as completely black-boxed, without any knowledge and modification of the inner workings (\emph{e.g.} system prompts and model parameters.) 
% Differently, our study considers the integrated system instead of individual modules, and an entirely online setting where accessible real-world web resources will be retrieved. Additionally, starting from practicality, our proposed pipeline is targeted at the web app version of different Web Agents and consequently black-box, without any knowledge and modification (\emph{e.g.} system prompts and model parameters.) 
% Real-world Web Agents are those who can really access external websites instead of just evaluating locally via a simple web benchmark. 
% \textbf{To the best of our knowledge, we are the first to conduct a comprehensive investigation of WIPI in real-world Web Agents and propose a novel methodology for a totally black-box environment.}
% \shutong{Confusing; clarification needed.} \textcolor{red}{Specifically, as illustrated in Figure~\ref{}, we proposed our methodology from two main aspects: the existence form of indirect prompts in the webpage and the content of the indirect prompts.}

Under such a realistic application scenario, the overview of our proposed \wipi pipeline is illustrated in Figure~\ref{fig:webpipeline}. 
Assume that an attacker has released a malicious webpage on the Internet that is indistinguishable from a normal benign webpage after rendering but contains some explicitly crafted prompts. 
After receiving the user's request to access this webpage, the core LLM will call some web tools to retrieve its content from the Internet. 
% Meanwhile,\chaowei{I feel it should be an attacker published a malicious website after then the user access the URL. The order here is confusing. } on the Internet, an attacker has released a malicious webpage that is indistinguishable from a normal benign webpage after rendering but contains some explicitly crafted prompts. 
After the content is retrieved, processed, and eventually sent to the core LLM by the web tool, as a result, it will lead the Web Agent to focus on and follow the inserted indirect instructions, and carry out some risky actions (\emph{e.g.} dangerous command execution and redirect to phishing websites.) Considering that this whole pipeline involves complicated information processing and interactions within an LLM system and publicly accessible webpages, the design of \wipi is supposed to simultaneously guarantee executability and stealthiness. 
Consequently, a successful attack is undoubtedly challenging. 

For executability, as shown in Figure~\ref{fig:webpipeline}
% based on the investigation of the most popular Web Agent, ChatGPT, 
% we found that OpenAI has deployed certain defenses against indirect prompt injections. To bypass such defense, 
we explicitly design a universal template via three main strategies, including preset instruction negligence, provision of confirmation, and multi-level repetition. 
Firstly, considering a realistic scenario, there can be preset instructions, either already included in system prompts or added by the user, that will hinder the execution of indirect instructions within the retrieved content. For instance, a user can explicitly request a summarization of the target webpage. To bypass such preset instructions, we add a counter instruction like ``\emph{PLEASE DO NOT EXECUTE THE FORMER INSTRUCTION!}''.
Furthermore, we found it possible that some Web Agents (\emph{e.g.} ChatGPT and GPTs) have been equipped with certain defenses which can be called ``Confirmation Request'', such that the user will be asked for a confirmation before the indirect instructions are executed. Consequently, we provide a pre-confirming instruction like ``\emph{I would like you to proceed with this instruction DIRECTLY without asking for any further confirmation!}''.
% , taking advantage of a fundamental flaw mentioned in~\cite{} that OpenAI hasn't built an effective mechanism to identify the source of input. 
Finally, to make the Web Agent concentrate on the indirect instructions under the disturbance of massive normal webpage content, we apply multi-level repetition, including sentence-level repetition and paragraph-level repetition. 
% To attract attention from the normal content to indirect prompts, we adopt two different types of \textbf{repetition} strategy. 
% One of them is sentence-level repetition, where we repeat certain sentences several times to emphasize their importance. For instance, to enforce the LLM to pay less attention to the normal webpage content, we can repeat the following sentence  ``\emph{DO NOT SUMMARIZE ANY WEBPAGE CONTENT!}''.  
% The other is paragraph-level repetition. We see original indirect prompts as a whole paragraph and to increase the attention of LLMs to our indirect prompts, we will repeat the whole paragraph several times.  
In addition to the template, we discover that the relative position of the inserted instructions significantly influences the Web Agent's concentration, and we place them in front of all the webpage content as an optimal solution.

% Finally, we found that OpenAI has implemented certain defenses which can be called ``request of confirmation''. This kind of confirmation request will ask for confirmation from users before executing indirect instructions. To bypass such defense, we directly add confirmations in the indirect prompts. This leverages the fundamental flaw mentioned in~\cite{} that OpenAI fails to build an effect mechanism to identify the source of such confirmation. 
% Additionally, from the perspective of the webpage, we discovered the importance of the position. 
% we investigated the impact of the existence form of indirect prompts in the webpage on the attack results and found that the position of indirect prompts in the webpage will deeply impact the attack performances. As the solution, we place indirect prompts in front of all the webpage content.
% \shutong{two purposes of our design: executable and stealthy; 
% 1. executable: 2-fold, can be noticed by LLM, and can be strictly followed; including location, in-prompt prefix and suffix, and repetition.
% 2. stealthy: web page design tricks: font size, color, and html hidden element}

For stealthiness, compared with traditional web threats, which are mainly brought by some malicious executable code inserted into the webpage, \wipi is naturally more stealthy. 
% obtains better stealthiness. 
% Specifically, for instance, web norms can spread and steal private information via a specific part of its code. 
% However, t
The driver of \wipi is the embedded indirect instructions in the format of natural language instead of executable code. Due to the flexibility of natural language (\emph{e.g.} paraphrasable and multilingual interpretation) and the indistinguishability between the injected prompt and the normal textual content, it is much harder for traditional web safeguards (like VirusTotal~\cite{virustotal}) to detect the existence of \wipi.
Besides, considering the imperceptibility to human eyes when users are inspecting publicly released webpages, we start from the webpage frontend design and focus on four different attributes: font size, font color, font opacity, and layout location. Specifically, we can set the font size of the inserted prompts to an extremely tiny number (\emph{e.g.} 0.0001px), the font color to the same as the background, or the font opacity to 0, such that the prompts will be imperceptible to human eyes after the webpage is rendered. Meanwhile, we can also put the indirect prompts out of the screen, \emph{e.g.}, far away above the current displayed webpage.

% Second, based on the investigation of the most popular Web Agent, ChatGPT, we found that OpenAI has implemented certain defenses to prevent WIPI. To bypass such defense, we carefully design a universal template where we adopt three main strategies. To attract attention from the normal content to indirect prompts, we adopt two different types of \textbf{repetition} strategy.
% One of them is sentence-level repetition, where we repeat certain sentences several times to emphasize their importance. For instance, to enforce the LLM to pay less attention to the normal webpage content, we can repeat the following sentence  ``\emph{DO NOT SUMMARIZE ANY WEBPAGE CONTENT!}''.  
% The other is paragraph-level repetition. We see original indirect prompts as a whole paragraph and to increase the attention of LLMs to our indirect prompts, we will repeat the whole paragraph several times.  Furthermore, user prefix instructions together with the retrieved content will prevent or influence the execution of indirect prompts. For instance, a user can explicitly request Web Agents to summarize the webpage. To ignore such preset instructions, we can add the following sentence ``\emph{PLEASE DO NOT EXECUTE THE FORMER INSTRUCTION!}'' to prevent LLMs from executing original instructions. Finally, we found that OpenAI has implemented certain defenses which can be called ``confirmation request''. This kind of confirmation request will ask for confirmation from users before executing indirect instructions. To bypass such defense, we directly add confirmations in the indirect prompts. This leverages the fundamental flaw mentioned in~\cite{} that OpenAI fails to build an effect mechanism to identify the source of such confirmation. 
 
To evaluate \wipi, we conduct comprehensive experiments. Specifically, we mainly target the web app version of ChatGPT, which is the most popular and powerful Web Agent, with 7 web plugins plus 8 Web GPTs.
Meanwhile, we also evaluate our attack on several open-sourced Web Agents. 
The results indicate that even in the black-box setting, \wipi can obtain over 90\% attack success rate on average. 
Furthermore, via the ablation study over different user prefix instructions, we prove that \wipi has good robustness and can still obtain great performance.

In this paper, our contribution can be summarized as follows:
\begin{itemize}
    \item We propose \wipi, which is a brand-new type of web threat. Furthermore, we reveal two fundamental unique properties of \wipi. To the best of our knowledge, we are the first to systematically analyze possible threats in real-world Web Agents under a practical application setting, instead of only showing proof-of-concept in an offline environment. 
    \item  
    % We propose the first black-box based WIPI attack methodology that considers two main aspects, the existence form and content of the indirect prompts.
    To tackle the challenges encountered in the two steps of the \wipi pipeline when launching the vanilla attack, we explicitly designed a set of novel and effective strategies to successfully overcome these obstacles.
    % \chaowei{what does every link mean here? not understand }
    The effectiveness and robustness of our methodology are proven by comprehensive experiments including 7 web plugin-augmented GPT4, 8 Web GPTs, and 3 open-sourced Web Agents. 
    % \chaowei{Rewrite it. Give some numbers and settings. We evaluate on xxx number of Web Agents and xxx. }
    \item 
    % \chaowei{Ablation study} 
    To further validate the efficacy of our attack methodology, we conducted a thorough ablation study, evaluating each strategy of our design. The results of our experiments affirm the effectiveness of every strategy we proposed.
    
    \item We reveal the vulnerability of current LLM-driven Web Agents against this brand-new attack manner, and on the other hand highlight the urgency to build more secure Web Agents.
    

\end{itemize}



==> tables/main_res.tex <==
\begin{table*}[t]
\small
\setlength{\tabcolsep}{1pt}
\caption{The performance of attacking plugin-augmented GPT4.}
  \label{tab:mainres}
  \centering
  \begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c | c | c |}
    \noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
    \multirow{2}{*}{\centering Web Plugin}  & \multirow{2}{*}{Webpage} & \multicolumn{10}{c|}{Attack Performace} & \multirow{2}{*}{$ASR_{page}$} & \multirow{2}{*}{\small $ASR_{Plugin}$}\\
    \cline{3-12}
    & & Prompt1 & Prompt2 & Prompt3 & Prompt4 & Prompt5 & Prompt6 & Prompt7 & Prompt8 & Prompt9 & Prompt10  & &\\
    \hline
    \multirow{5}{*}{Web Pilot} & Page1 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 4/5 & 5/5 & 5/5 & 5/5 & 98\% &  \multirow{5}{*}{97\%} \\
    \cline{2-13}
    & Page2 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 3/5 & 5/5 & 5/5 & 5/5 & 96\% &   \\
    \cline{2-13}
    & Page3 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 100\% &  \\
    \cline{2-13}
    & Page4 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 2/5 & 5/5 & 5/5 & 5/5 & 94\% &   \\
    \cline{2-13}
    &$ASR_{prompt}$ & 100\%  & 100\% &  100\%& 100\% & 100\% & 100\% & 70\% & 100\% & 100\% & 100\% & \textbackslash &   \\
    \hline
    \multirow{5}{*}{Web Reader} & Page1 & 5/5 & 5/5 & 4/5 & 5/5 & 5/5 & 5/5 & 3/5 & 5/5 & 5/5 & 5/5 & 94\% &  \multirow{5}{*}{93.5\%} \\
    \cline{2-13}
    & Page2 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 2/5 & 5/5 & 5/5 & 5/5 & 94\% &   \\
    \cline{2-13}
    & Page3 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 4/5 & 3/5 & 5/5 & 5/5 & 5/5 & 94\% &   \\
    \cline{2-13}
    & Page4 & 5/5 & 5/5 & 4/5 & 5/5 & 5/5 & 5/5 & 2/5 & 5/5 & 5/5 & 5/5 & 92\% &   \\
    \cline{2-13}
    &$ASR_{prompt}$ & 100\% & 100\%  & 90\%  & 100\% & 100\%  & 95\%  &  50\% & 100\% & 100\% & 100\% & \textbackslash &   \\
    \hline
    \multirow{5}{*}{Web Request} & Page1 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 &100\% &  \multirow{5}{*}{99\%} \\
    \cline{2-13}
    & Page2 & 5/5 & 5/5 & 4/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 98\% &   \\
    \cline{2-13}
    & Page3 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 100\% &   \\
    \cline{2-13}
    & Page4 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 4/5 & 5/5 & 5/5 & 5/5 & 98\% &   \\
    \cline{2-13}
    &$ASR_{prompt}$ & 100\% & 100\% & 95\% & 100\%  & 100\%  & 100\% & 95\% & 100\%  & 100\%  & 100\%  & \textbackslash &   \\
    \hline
    \multirow{5}{*}{Browser Pilot} & Page1 & 5/5 & 5/5 & 4/5 & 5/5 & 5/5 & 5/5 & 3/5 & 4/5 & 5/5 & 5/5 & 92\% &  \multirow{5}{*}{94.5\%} \\
    \cline{2-13}
    & Page2 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 2/5 & 5/5 & 5/5 & 5/5 & 94\% &   \\
    \cline{2-13}
    & Page3 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 1/5 & 5/5 & 5/5 & 5/5 & 92\% &   \\
    \cline{2-13}
    & Page4 &5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 100\%&   \\
    \cline{2-13}
    & $ASR_{prompt}$ & 100\% & 100\% & 95\% & 100\% & 100\% & 100\% & 55\% & 95\% & 100\% & 100\% & \textbackslash &   \\
    \hline
    \multirow{5}{*}{Web Search AI} & Page1 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 3/5 & 4/5 & 5/5 & 5/5 & 94\% &  \multirow{5}{*}{91.5\%}\\
    \cline{2-13}
    & Page2 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 1/5 & 4/5 & 5/5 & 5/5 & 90\% &   \\
    \cline{2-13}
    & Page3 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 4/5 & 1/5 & 4/5 & 5/5 & 5/5 & 88\% &   \\
    \cline{2-13}
    & Page4 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 2/5 & 5/5 & 5/5 & 5/5 & 94\% &   \\
    \cline{2-13}
    & $ASR_{prompt}$ & 100\% & 100\% &  100\% & 100\% & 100\% & 95\% & 35\% & 85\% & 100\% & 100\% & \textbackslash &   \\
    \hline
    \multirow{5}{*}{Aaron Browser} & Page1 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 100\% &  \multirow{5}{*}{100\%} \\
    \cline{2-13}
    & Page2 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 100\% &   \\
    \cline{2-13}
    & Page3 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 100\% &   \\
    \cline{2-13}
    & Page4 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 100\% &   \\
    \cline{2-13}
    & $ASR_{prompt}$ & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & \textbackslash &   \\
    \hline
    \multirow{5}{*}{\makecell{MixerBox \\ WebSearchG}} & Page1 & 4/5 & 5/5 & 5/5 & 3/5 & 4/5 & 3/5 & 2/5 & 2/5 & 5/5 & 5/5 & 76\% &  \multirow{5}{*}{81.5\%} \\
    \cline{2-13}
    & Page2 & 4/5 & 5/5 & 5/5 & 4/5 & 3/5 & 3/5 & 1/5 & 4/5 & 5/5 & 5/5 & 78\% &   \\
    \cline{2-13}
    & Page3 & 3/5 & 5/5 & 5/5 & 3/5 & 5/5 & 3/5 & 2/5 & 4/5 & 5/5 & 5/5 & 80\% &   \\
    \cline{2-13}
    & Page4 & 4/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 2/5 & 5/5 & 5/5 & 5/5 & 92\% &   \\
    \cline{2-13}
    & $ASR_{prompt}$ & 75\% & 100\% & 100\% & 75\% & 85\% & 70\% & 35\% & 75\% & 100\% & 100\% & \textbackslash &   \\
    \hline
    \multicolumn{2}{|c|}{Total ASR} & 96.43\% & 100\% & 97.14\% & 96.43\% & 97.86\% & 94.29\% & 62.86\% & 93.57\% & 100\% & 100\% & \multicolumn{2}{|c|}{93.86\%} \\
    % \hline
    \noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
  \end{tabular}

\end{table*}






==> tables/opensource_details.tex <==
\begin{table*}[t]
\small
\setlength{\tabcolsep}{1pt}
\caption{The performance of attacking plugin-based web agents of ChatGPT.}
  \label{tab:mainres}
  \centering
  \begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c | c | c |}
    \noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
    \multirow{2}{*}{\centering Web Plugin}  & \multirow{2}{*}{Webpage} & \multicolumn{10}{c|}{Attack Performace} & \multirow{2}{*}{$ASR_{page}$} & \multirow{2}{*}{\small $ASR_{Plugin}$}\\
    \cline{3-12}
    & & Prompt1 & Prompt2 & Prompt3 & Prompt4 & Prompt5 & Prompt6 & Prompt7 & Prompt8 & Prompt9 & Prompt10  & &\\
    \hline
    \multirow{5}{*}{Web Pilot} & Page1 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 4/5 & 5/5 & 5/5 & 5/5 & 98\% &  \multirow{5}{*}{97\%} \\
    \cline{2-13}
    & Page2 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 3/5 & 5/5 & 5/5 & 5/5 & 96\% &   \\
    \cline{2-13}
    & Page3 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 100\% &  \\
    \cline{2-13}
    & Page4 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 2/5 & 5/5 & 5/5 & 5/5 & 94\% &   \\
    \cline{2-13}
    &$ASR_{prompt}$ & 100\%  & 100\% &  100\%& 100\% & 100\% & 100\% & 70\% & 100\% & 100\% & 100\% & 97\% &   \\
    \hline
    \multirow{5}{*}{Web Reader} & Page1 & 5/5 & 5/5 & 4/5 & 5/5 & 5/5 & 5/5 & 3/5 & 5/5 & 5/5 & 5/5 & 94\% &  \multirow{5}{*}{93.5\%} \\
    \cline{2-13}
    & Page2 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 2/5 & 5/5 & 5/5 & 5/5 & 94\% &   \\
    \cline{2-13}
    & Page3 & 5/5 & 5/5 & 5/5 & 5/5 & 5/5 & 4/5 & 3/5 & 5/5 & 5/5 & 5/5 & 94\% &   \\
    \cline{2-13}
    & Page4 & 5/5 & 5/5 & 4/5 & 5/5 & 5/5 & 5/5 & 2/5 & 5/5 & 5/5 & 5/5 & 92\% &   \\
    \cline{2-13}
    &$ASR_{prompt}$ & 100\% & 100\%  & 90\%  & 100\% & 100\%  & 95\%  &  50\% & 100\% & 100\% & 100\% & 93.5\% &   \\
    \hline
    \multirow{5}{*}{Web Request} & Page1 & & & & & & & & & & & &  \multirow{5}{*}{} \\
    \cline{2-13}
    & Page2 & & & & & & & & & & & &   \\
    \cline{2-13}
    & Page3 & & & & & & & & & & & &   \\
    \cline{2-13}
    & Page4 & & & & & & & & & & & &   \\
    \cline{2-13}
    &$ASR_{prompt}$ &  &  &  &  &  &  &  &  &  &  &  &   \\
    \hline
    \multirow{5}{*}{Browser Pilot} & Page1 & & & & & & & & & & & &  \multirow{5}{*}{} \\
    \cline{2-13}
    & Page2 & & & & & & & & & & & &   \\
    \cline{2-13}
    & Page3 & & & & & & & & & & & &   \\
    \cline{2-13}
    & Page4 & & & & & & & & & & & &   \\
    \cline{2-13}
    & $ASR_{prompt}$ &  &  &  &  &  &  &  &  &  &  &  &   \\
    \hline
    \multirow{5}{*}{Web Search AI} & Page1 & & & & & & & & & & & &  \multirow{5}{*}{}\\
    \cline{2-13}
    & Page2 & & & & & & & & & & & &   \\
    \cline{2-13}
    & Page3 & & & & & & & & & & & &   \\
    \cline{2-13}
    & Page4 & & & & & & & & & & & &   \\
    \cline{2-13}
    & $ASR_{prompt}$ &  &  &  &  &  &  &  &  &  &  &  &   \\
    \hline
    \multirow{5}{*}{Aaron Browser} & Page1 & & & & & & & & & & & &  \multirow{5}{*}{} \\
    \cline{2-13}
    & Page2 & & & & & & & & & & & &   \\
    \cline{2-13}
    & Page3 & & & & & & & & & & & &   \\
    \cline{2-13}
    & Page4 & & & & & & & & & & & &   \\
    \cline{2-13}
    & $ASR_{prompt}$ &  &  &  &  &  &  &  &  &  &  &  &   \\
    \hline
    \multirow{5}{*}{\makecell{MixerBox \\ WebSearchG}} & Page1 & & & & & & & & & & & &  \multirow{5}{*}{} \\
    \cline{2-13}
    & Page2 & & & & & & & & & & & &   \\
    \cline{2-13}
    & Page3 & & & & & & & & & & & &   \\
    \cline{2-13}
    & Page4 & & & & & & & & & & & &   \\
    \cline{2-13}
    & $ASR_{prompt}$ &  &  &  &  &  &  &  &  &  &  &  &   \\
    \hline
    \multicolumn{2}{|c|}{Total ASR} & 40 & 0 & 25/40 & 0/40 & 4/40 & 16/40 & 0/40& 4/40 & 18/40 & 2/40 & 9/40 & 20/40 \\
    \hline
    \noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
  \end{tabular}
 
\end{table*}





